Toward Ambulatory Vision: Learning Visually-Grounded Active View Selection

Vision Language Models (VLMs) excel at visual question answering (VQA) but remain limited to snapshot vision, reasoning from static images. In contrast, embodied agents require ambulatory vision, actively moving to obtain more informative views. We introduce Visually Grounded Active View Selection (VG-AVS), a task that selects the most informative next viewpoint using only the visual information in the current image, without relying on scene memory or external knowledge. To support this task, we construct a synthetic dataset with automatically generated paired query-target views and question-answer prompts. We also propose a framework that fine-tunes pretrained VLMs through supervised fine-tuning (SFT) followed by RL-based policy optimization. Our approach achieves strong question answering performance based on viewpoint selection and generalizes robustly to unseen synthetic and real scenes. Furthermore, incorporating our learned VG-AVS framework into existing scene-exploration-based EQA systems improves downstream question-answering accuracy.

==> figures/quali_benchmark_partial.tex <==
% Preamble (once)
% \usepackage{graphicx,booktabs,tabularx,array,xcolor}
% \newcolumntype{Y}{>{\centering\arraybackslash}X}
% \setlength{\tabcolsep}{1pt}
% preamble

%\definecolor{wrongblue}{RGB}{38,82,170}
%\definecolor{correctred}{RGB}{192,57,43}

% \definecolor{correctgreen}{RGB}{105,182,28}
% \definecolor{wrongred}{RGB}{243,43,12}
% \definecolor{correctgreen}{RGB}{132,153,79}
% \definecolor{wrongred}{RGB}{243,1,3}

\definecolor{correctgreen}{RGB}{26,187,46}
\definecolor{wrongred}{RGB}{243,1,3}



\newcommand{\imgframe}[2]{
\begingroup \setlength{\fboxsep}{0pt}
\setlength{\fboxrule}{1.3pt}% 테두리 두께 (원하면 조절) 
\fcolorbox{#1}{white}{\includegraphics[width=1.0\linewidth,keepaspectratio]{#2}}% 
\endgroup }

% \newcommand{\imgframe}[2]{%
%   \tcbox[colframe=#1, colback=white,
%          boxrule=1.3pt, boxsep=0pt,
%          arc=3pt,    % 모서리 라운드 정도
%          enhanced]{%
%     \includegraphics[width=0.96\linewidth,keepaspectratio]{#2}%
%   }%
% }

\newcommand{\hcell}[1]{\makecell{\scriptsize #1}}
\begin{figure*}[t]
\scriptsize
\centering
\renewcommand{\arraystretch}{1.0}
\setlength{\tabcolsep}{1pt}
\arrayrulecolor{black}
\setlength{\arrayrulewidth}{0.2pt}

%\newcommand{\receptacle}[1]{\colorbox{gray!15}{\strut #1}}
\newcommand{\receptacle}[1]{%
  \begingroup
  \setlength{\fboxsep}{2pt}% 기본값(3pt)보다 훨씬 작게
  \colorbox{olive!15}{#1}%
  \endgroup
}
\newcommand{\targetobj}[1]{%
  \begingroup
  \setlength{\fboxsep}{2pt}% 기본값(3pt)보다 훨씬 작게
  \colorbox{blue!15}{#1}%
  \endgroup
}


\newcommand{\wrongimg}[2][]{%
  \begin{overpic}[#1]{#2}
    \put(3,75){\color{wrongred}\fontsize{15}{15}\selectfont\bfseries\xmark}
  \end{overpic}
}

\newcommand{\correctimg}[2][]{%
  \begin{overpic}[#1]{#2}
    \put(3,75){\color{correctgreen}\fontsize{15}{15}\selectfont\bfseries\cmark}
  \end{overpic}
}


\begin{tabularx}{\linewidth}{YYYYYYYYY}
\toprule
% ===== Category header row =====
& \multicolumn{1}{c|}{} & \hcell{EQA\\Framework} & \hcell{Backbone\\Model} & \hcell{Proprietary\\Model} & \hcell{Spatial\\VLM} & \multicolumn{3}{|c}{\hcell{AVS Framework}} \\
\midrule
% ===== Model-name header row (no bold, smaller font) =====
Query View & \multicolumn{1}{c|}{Target View} & \hcell{Fine-EQA~\cite{Liu:2024EXPRESSBench}} & \hcell{Qwen-2.5-VL~\cite{Bai:2025Qwen2.5VL}} & \hcell{Gemini-2.5\\-Pro~\cite{Google:2025Gemini25}} & \hcell{ViLaSR~\cite{Junfei:2025VILASR}} & \multicolumn{1}{|c}{\hcell{SFT}} & \hcell{RL} & \hcell{\textbf{SFT+RL (Ours)}} \\
\midrule
%\multicolumn{9}{c}{\Benchmark{}-ProcTHOR}
%\midrule
% ---- Rows (GPT / VILA-SR set) ----
%\RowNine{figures/quali_cropped/procthor/counting_gpt_vilasr_0063}{(Counting) ``\textit{ How many \textbf{cups} on the \textbf{sofa}?}''}
\multicolumn{9}{c}{\footnotesize (Counting) ``\textit{How many \targetobj{\textbf{mugs}} near the \receptacle{\textbf{diningtable}}?}''}\\[4pt]
\includegraphics[width=\linewidth,keepaspectratio]{figures/quali_cropped/procthor/counting_gemini_vilasr_0478/input.png} &
\includegraphics[width=\linewidth,keepaspectratio]{figures/quali_cropped/procthor/counting_gemini_vilasr_0478/gt.png} &
\wrongimg[width=\linewidth,keepaspectratio]{{figures/quali_cropped/procthor/counting_gemini_vilasr_0478/eqa.png}} &
\wrongimg[width=\linewidth,keepaspectratio]{{figures/quali_cropped/procthor/counting_gemini_vilasr_0478/qwen.png}} &
\wrongimg[width=\linewidth,keepaspectratio]{{figures/quali_cropped/procthor/counting_gemini_vilasr_0478/pro.png}} &
\wrongimg[width=\linewidth,keepaspectratio]{{figures/quali_cropped/procthor/counting_gemini_vilasr_0478/spatial.png}} &
\correctimg[width=\linewidth,keepaspectratio]{{figures/quali_cropped/procthor/counting_gemini_vilasr_0478/sft.png}} &
\correctimg[width=\linewidth,keepaspectratio]{{figures/quali_cropped/procthor/counting_gemini_vilasr_0478/grpo.png}} &
\correctimg[width=\linewidth,keepaspectratio]{{figures/quali_cropped/procthor/counting_gemini_vilasr_0478/ours_marked.png}} \\

\midrule
%\RowNine{figures/quali_cropped/procthor/state_gpt_vilasr_0366}{(State) ``\textit{Choose a \textbf{toiletpaper}'s state on the \textbf{toilet}. A: used up. B: unused.}''}
\multicolumn{9}{c}{\footnotesize (State) ``\textit{Choose a \targetobj{\textbf{toiletpaper}}'s state on the \receptacle{\textbf{toilet}}. A: used up. B: unused.}''}\\[4pt]
\includegraphics[width=\linewidth,keepaspectratio]{figures/quali_cropped/procthor/state_gemini_vilasr_0366/input.png} &
\includegraphics[width=\linewidth,keepaspectratio]{figures/quali_cropped/procthor/state_gemini_vilasr_0366/gt.png} &
\wrongimg[width=\linewidth,keepaspectratio]{{figures/quali_cropped/procthor/state_gemini_vilasr_0366/eqa.png}} &
\wrongimg[width=\linewidth,keepaspectratio]{{figures/quali_cropped/procthor/state_gemini_vilasr_0366/qwen.png}} &
\correctimg[width=\linewidth,keepaspectratio]{{figures/quali_cropped/procthor/state_gemini_vilasr_0366/pro.png}} &
\wrongimg[width=\linewidth,keepaspectratio]{{figures/quali_cropped/procthor/state_gemini_vilasr_0366/spatial.png}} &
\correctimg[width=\linewidth,keepaspectratio]{{figures/quali_cropped/procthor/state_gemini_vilasr_0366/sft.png}} &
\correctimg[width=\linewidth,keepaspectratio]{{figures/quali_cropped/procthor/state_gemini_vilasr_0366/grpo.png}} & 
\correctimg[width=\linewidth,keepaspectratio]{{figures/quali_cropped/procthor/state_gemini_vilasr_0366/ours_marked.png}} \\

\midrule
%\RowNine{figures/quali_cropped/procthor/state_gpt_vilasr_0366}{(State) ``\textit{Choose a \textbf{toiletpaper}'s state on the \textbf{toilet}. A: used up. B: unused.}''}
\multicolumn{9}{c}{\footnotesize (State) ``\textit{Choose a \targetobj{\textbf{laptop}}'s state on the \receptacle{\textbf{desk}}. A: opened. B: closed.}''}\\[4pt]
\includegraphics[width=\linewidth,keepaspectratio]{figures/quali_cropped/procthor/state_gemini_vilasr_0021/input.png} &
\includegraphics[width=\linewidth,keepaspectratio]{figures/quali_cropped/procthor/state_gemini_vilasr_0021/gt.png} &
\wrongimg[width=\linewidth,keepaspectratio]{{figures/quali_cropped/procthor/state_gemini_vilasr_0021/eqa.png}} &
\wrongimg[width=\linewidth,keepaspectratio]{{figures/quali_cropped/procthor/state_gemini_vilasr_0021/qwen.png}} &
\wrongimg[width=\linewidth,keepaspectratio]{{figures/quali_cropped/procthor/state_gemini_vilasr_0021/pro.png}} &
\wrongimg[width=\linewidth,keepaspectratio]{{figures/quali_cropped/procthor/state_gemini_vilasr_0021/spatial.png}} &
\correctimg[width=\linewidth,keepaspectratio]{{figures/quali_cropped/procthor/state_gemini_vilasr_0021/sft.png}} &
\correctimg[width=\linewidth,keepaspectratio]{{figures/quali_cropped/procthor/state_gemini_vilasr_0021/grpo.png}} & 
\correctimg[width=\linewidth,keepaspectratio]{{figures/quali_cropped/procthor/state_gemini_vilasr_0021/ours_marked.png}} \\

\midrule
%\multicolumn{9}{c}{\Benchmark{}-HM3D}
%\midrule
%\RowNine{figures/quali_cropped/hm3d/gpt_vilasr_0165}{(State) ``\textit{Is the \textbf{lamp} in the bedroom next to the window \textbf{turned on}?}''}

% ===== Category header row for second block (Gemini / SpatialReasoner) =====
% ===== Model-name header row variant (Gemini / SpatialReasoner) =====
%\hcell{Query View} & \hcell{Target View} & \hcell{Fine-EQA~\cite{Liu:2024EXPRESSBench}} & \hcell{Qwen-2.5-VL~\cite{Bai:2025Qwen2.5VL}} & \hcell{Gemini-2.5\\Pro~\cite{Google:2025Gemini25}} & \hcell{Spatial\\ Reasoner~\cite{Ma:2025SpatialReasoner}} & \hcell{SFT} & \hcell{RL} & \hcell{\textbf{Ours}} \\
%\midrule 
% ---- Rows (Gemini / SpatialReasoner set) ----
%\RowNine{figures/quali_cropped/procthor/counting_gemini_spatialreasoner_0478}{(Counting) ``\textit{How many \textbf{mugs} near the \textbf{diningtable}?}''}

\multicolumn{9}{c}{\footnotesize (Counting) ``\textit{How many \targetobj{\textbf{paintings}} are hanging on the wall near the \receptacle{\textbf{sofa}} in the living room?}''}\\[4pt]
\includegraphics[width=\linewidth,keepaspectratio]{figures/quali_cropped/hm3d/gemini_vilasr_0042/input.png} &
\includegraphics[width=\linewidth,keepaspectratio]{figures/quali_cropped/hm3d/gemini_vilasr_0042/gt.png} &
%\fcolorbox{blue}{white}
\wrongimg[width=\linewidth,keepaspectratio]{{figures/quali_cropped/hm3d/gemini_vilasr_0042/eqa.png}} &
\wrongimg[width=\linewidth,keepaspectratio]{{figures/quali_cropped/hm3d/gemini_vilasr_0042/qwen.png}} &
\correctimg[width=\linewidth,keepaspectratio]{{figures/quali_cropped/hm3d/gemini_vilasr_0042/pro.png}} &
\wrongimg[width=\linewidth,keepaspectratio]{{figures/quali_cropped/hm3d/gemini_vilasr_0042/spatial.png}} &
\correctimg[width=\linewidth,keepaspectratio]{{figures/quali_cropped/hm3d/gemini_vilasr_0042/sft.png}} &
\correctimg[width=\linewidth,keepaspectratio]{{figures/quali_cropped/hm3d/gemini_vilasr_0042/grpo.png}} &
\correctimg[width=\linewidth,keepaspectratio]{{figures/quali_cropped/hm3d/gemini_vilasr_0042/ours_marked.png}} \\

\midrule

\multicolumn{9}{c}{\footnotesize (Existence) ``\textit{Is there a \targetobj{\textbf{space}} for my winter coat in the \receptacle{\textbf{closet}} in the cloakroom?}''}\\[4pt]
\includegraphics[width=\linewidth,keepaspectratio]{figures/quali_cropped/hm3d/gemini_vilasr_0093/input.png} &
\includegraphics[width=\linewidth,keepaspectratio]{figures/quali_cropped/hm3d/gemini_vilasr_0093/gt.png} &
\correctimg[width=\linewidth,keepaspectratio]{{figures/quali_cropped/hm3d/gemini_vilasr_0093/eqa.png}} &
\wrongimg[width=\linewidth,keepaspectratio]{{figures/quali_cropped/hm3d/gemini_vilasr_0093/qwen.png}} &
\wrongimg[width=\linewidth,keepaspectratio]{{figures/quali_cropped/hm3d/gemini_vilasr_0093/pro.png}} &
\wrongimg[width=\linewidth,keepaspectratio]{{figures/quali_cropped/hm3d/gemini_vilasr_0093/spatial.png}} &
\correctimg[width=\linewidth,keepaspectratio]{{figures/quali_cropped/hm3d/gemini_vilasr_0093/sft.png}} &
\correctimg[width=\linewidth,keepaspectratio]{{figures/quali_cropped/hm3d/gemini_vilasr_0093/grpo.png}} &
\correctimg[width=\linewidth,keepaspectratio]{{figures/quali_cropped/hm3d/gemini_vilasr_0093/ours_marked.png}}
\\

% \multicolumn{9}{c}{\footnotesize (State) ``\textit{Did I hang up the \targetobj{\textbf{paintings}} in the \receptacle{\textbf{hallway}}?}''}\\[4pt]
% \includegraphics[width=\linewidth,keepaspectratio]{figures/quali_cropped/hm3d/gemini_vilasr_0201/input.png} &
% \includegraphics[width=\linewidth,keepaspectratio]{figures/quali_cropped/hm3d/gemini_vilasr_0201/gt.png} &
% \wrongimg[width=\linewidth,keepaspectratio]{{figures/quali_cropped/hm3d/gemini_vilasr_0201/eqa.png}} &
% \wrongimg[width=\linewidth,keepaspectratio]{{figures/quali_cropped/hm3d/gemini_vilasr_0201/qwen.png}} &
% \wrongimg[width=\linewidth,keepaspectratio]{{figures/quali_cropped/hm3d/gemini_vilasr_0201/pro.png}} &
% \wrongimg[width=\linewidth,keepaspectratio]{{figures/quali_cropped/hm3d/gemini_vilasr_0201/spatial.png}} &
% \correctimg[width=\linewidth,keepaspectratio]{{figures/quali_cropped/hm3d/gemini_vilasr_0201/sft.png}} &
% \correctimg[width=\linewidth,keepaspectratio]{{figures/quali_cropped/hm3d/gemini_vilasr_0201/grpo.png}} &
% \correctimg[width=\linewidth,keepaspectratio]{{figures/quali_cropped/hm3d/gemini_vilasr_0201/ours_marked.png}}\\
\midrule

\multicolumn{9}{c}{\footnotesize (State) ``\textit{Is the \targetobj{\textbf{lamp}} in the bedroom next to the \receptacle{\textbf{window}} turned on?}''}\\[4pt]
\includegraphics[width=\linewidth,keepaspectratio]{figures/quali_cropped/hm3d/gpt_vilasr_0165/input.png} &
\includegraphics[width=\linewidth,keepaspectratio]{figures/quali_cropped/hm3d/gpt_vilasr_0165/gt.png} &
\wrongimg[width=\linewidth,keepaspectratio]{{figures/quali_cropped/hm3d/gpt_vilasr_0165/eqa.png}} &
\wrongimg[width=\linewidth,keepaspectratio]{{figures/quali_cropped/hm3d/gpt_vilasr_0165/qwen.png}} &
\wrongimg[width=\linewidth,keepaspectratio]{{figures/quali_cropped/hm3d/gpt_vilasr_0165/pro.png}} &
\wrongimg[width=\linewidth,keepaspectratio]{{figures/quali_cropped/hm3d/gpt_vilasr_0165/spatial.png}} &
\correctimg[width=\linewidth,keepaspectratio]{{figures/quali_cropped/hm3d/gpt_vilasr_0165/sft.png}} &
\correctimg[width=\linewidth,keepaspectratio]{{figures/quali_cropped/hm3d/gpt_vilasr_0165/grpo.png}} &
\correctimg[width=\linewidth,keepaspectratio]{{figures/quali_cropped/hm3d/gpt_vilasr_0165/ours_marked.png}} \\
% \midrule
\bottomrule
\end{tabularx}
\vspace{-\baselineskip}
\caption{\textbf{Qualitative results in \Benchmark{}-ProcTHOR (upper 3 rows) and \Benchmark{}-HM3D (lower 3 rows).} \targetobj{Blue} denotes object-of-interest, and \receptacle{gray} denotes visual clues used for reasoning. \correctmark corresponds to correct answers (or LLM-Match scores $\geq$ 5), \wrongmark corresponds to wrong answers (or LLM-Match scores $\leq$ 2). The red arrow in the final column marks the region of interest.}
\label{fig:quali_benchmark}
\vspace{-\baselineskip}
\end{figure*}


==> figures/thinking_images/backup/_fine-eqa_image_list.tex <==
\ImagePair{figures/thinking_images/fine-eqa_1.pdf}{figures/thinking_images/fine-eqa_3.pdf}
\ImagePair{figures/thinking_images/fine-eqa_6.pdf}{figures/thinking_images/fine-eqa_7.pdf}
\ImagePairLast{figures/thinking_images/fine-eqa_4.pdf}{figures/thinking_images/fine-eqa_5.pdf}

==> figures/thinking_images/backup/_hm3d_image_list.tex <==
\ImagePair{figures/thinking_images/hm_1.pdf}{figures/thinking_images/hm_2.pdf}
\ImagePair{figures/thinking_images/hm_3.pdf}{figures/thinking_images/hm_4.pdf}
\ImagePairLast{figures/thinking_images/hm_5.pdf}{figures/thinking_images/hm_6.pdf}

==> figures/thinking_images/backup/_hm3d_image_list_2.tex <==
\ImagePair{figures/thinking_images/hm_7.pdf}{figures/thinking_images/hm_8.pdf}
\ImagePairLast{figures/thinking_images/hm_9.pdf}{figures/thinking_images/hm_10.pdf}




==> figures/thinking_images/backup/_procthor_image_list.tex <==
\ImagePair{figures/thinking_images/procthor_1.pdf}{figures/thinking_images/procthor_2.pdf}
\ImagePair{figures/thinking_images/procthor_7.pdf}{figures/thinking_images/procthor_8.pdf}
\ImagePair{figures/thinking_images/procthor_5.pdf}{figures/thinking_images/procthor_6.pdf}
\ImagePairLast{figures/thinking_images/procthor_3.pdf}{figures/thinking_images/procthor_4.pdf}



==> figures/thinking_images/backup/_procthor_image_list_2.tex <==
\ImagePair{figures/thinking_images/procthor_5.pdf}{figures/thinking_images/procthor_6.pdf}
\ImagePair{figures/thinking_images/procthor_7.pdf}{figures/thinking_images/procthor_8.pdf}
\ImagePairLast{figures/thinking_images/procthor_9.pdf}{figures/thinking_images/procthor_10.pdf}




==> sec/1_intro_v1.tex <==
\section{Introduction}
\label{sec:intro}

Embodied question answering (EQA) with vision-language models (VLMs) has been a central topic in embodied AI, aiming to enable agents to perceive, reason, and act based on visual and linguistic inputs. Recent advancements have improved the visual understanding and language alignment capabilities of large VLMs, but their ability to perform spatially grounded reasoning—reasoning that depends on viewpoint and 3D context—remains limited.

A key limitation stems from the way existing EQA datasets are constructed. In most benchmarks, the agent is initialized from random viewpoints, regardless of the question being asked. This design overlooks an essential aspect of spatial reasoning: the agent’s need to interpret where it is and how to move to gather informative visual evidence. As a result, even powerful VLMs often fail to leverage geometric cues or actively seek better observations when the initial view provides incomplete information.

To address this gap, we introduce Last Mile Camera Calibration (LMCC), a new benchmark that emphasizes viewpoint-aware reasoning grounded in partial visual evidence. Our setting mimics how humans behave in similar circumstances: when faced with uncertainty due to occlusion or limited field of view, humans instinctively rotate their heads or shift positions to resolve ambiguity before answering a question. LMCC encourages VLM agents to exhibit this same form of adaptive exploration.

Unlike prior datasets that treat navigation as a means to reach target objects, LMCC formulates the problem as last-mile viewpoint calibration—the refinement of camera pose based on subtle visual clues. Given a partially informative observation, the agent must infer how to reposition itself to obtain a view that enables confident reasoning. This setup explicitly tests an agent’s ability to interpret geometric relations and to act according to those inferred cues.


We build LMCC using diverse scenes and question templates that induce partial observability and spatial ambiguity. The benchmark covers a wide range of camera configurations and environmental layouts, ensuring that improvement on LMCC reflects genuine enhancement in spatial reasoning rather than dataset-specific memorization. Through supervised and reinforcement fine-tuning on LMCC, VLMs learn to couple perception with viewpoint adjustment—a fundamental skill for grounded reasoning in 3D environments.

LMCC isolates the core embodied reasoning component—how an agent should refine its viewpoint when partial visual evidence already exists.
This “last-mile” setup evaluates visual geometry understanding and active calibration, not just goal-seeking.

We explore different parameterizations of action spaces, covering the full spectrum of 3D exploration while maintaining efficiency. The first is agent-centric, consisting of primitive actions such as rotate, move forward, and look, following the atomic actions prevalently used in EQA setups. Rotate adjusts the camera’s yaw and pitch angles in place, forward translates the agent along its current viewing direction, and look changes the camera orientation without changing position, allowing fine-grained viewpoint calibration. The second is human-centric, inspired by how humans reason spatially: the agent first estimates the target object (i.e., the center of the orbit) and then orbits around it to obtain a more informative viewpoint. We demonstrate that this human-centric action parameterization consistently outperforms its agent-centric counterpart.

Importantly, we show that models fine-tuned on LMCC not only perform better within the benchmark itself but also generalize to other spatial reasoning tasks, such as embodied navigation and 3D visual grounding. This demonstrates that our dataset cultivates a transferable inductive bias for spatially grounded understanding, serving as a crucial step toward embodied VLMs capable of reasoning through active perception.


\jk{Existing exploration methods's actions are constrained in the FoV of current viewpoint, while our action fully spans 3D environments.}



==> sec/1_intro_v2.tex <==
\section{Introduction}
\label{sec:intro}

\begin{flushright}
\begin{minipage}{0.91\linewidth}
\vspace{0.5em}
{
\itshape
``We look around, walk up to something interesting and move around it so as to see it from all sides, and go from one vista to another. That is natural vision.''
}
\vspace{0.5em}
\hrule height 0.4pt

\vspace{0.5em}
\hfill \textsc{James J. Gibson}~\cite{Gibson:1979Ecological}

\end{minipage}
\end{flushright}
% \begin{center}
% \begin{minipage}{0.9\linewidth}
% \vspace{0.5em}
% % \hrule height 0.6pt
% % \vspace{0.75em}
% \raggedright\itshape
% ``We look around, walk up to something interesting and move around it so as to see it from all sides, and go from one vista to another. That is natural vision.''

% \vspace{0.25em}
% \raggedleft\upshape---\textsc{James J. Gibson}
% \vspace{0.75em}
% \hrule height 0.6pt
% \vspace{0.5em}
% \end{minipage}
% \end{center}

% Over the past decade of research in Visual Question Answering (VQA), we have now witnessed the rise of Visual–Language Models (VLMs) that have essentially mastered the task, seemingly closing the chapter on this line of inquiry. What, then, should be the next step? We approach this question by revisiting the fundamental purpose of the visual system. James J. Gibson, one of the most influential psychologists of the 20th century, offered crucial insights through his \emph{ecological} approach to vision~\cite{Gibson:1979Ecological}.

We are now witnessing the rise of Visual–Language Models (VLMs) that have effectively mastered the Visual Question Answering (VQA) task, seemingly closing the chapter on this line of inquiry. What, then, should come next?

To explore this question, we revisit the fundamental purpose of vision itself. James J. Gibson, one of the most influential vision researchers of the 20th century, provided key insights through his \emph{ecological} approach to perception~\cite{Gibson:1979Ecological}. Current VLMs, despite their impressive capabilities, are confined to interpreting a single static image---a capacity Gibson termed “snapshot vision.” The early history of computer vision can similarly be viewed as the pursuit of this ability: understanding a retinal image. However, the true problem of vision in humans and animals lies beyond this static interpretation. As Gibson wrote, “natural vision depends on the eyes in the head on a body supported by the ground.” In other words, vision in the real world involves looking around, walking toward objects of interest, and observing them from multiple viewpoints---an ability he called “ambulatory vision.”

In this work, given a VQA problem and assuming an embodied agent situated within a scene, our goal is to fine-tune a VLM to select the most informative viewpoint for answering the question. Unlike prior active perception methods~\cite{} that rely on pre-memorized scene representations or external commonsense knowledge, our approach focuses on developing a system that operates purely based on the visual information available in the current observation. We refer to this task as Visually-Grounded Active View Selection (VG-AVS).

In recent computer vision research, the active perception systems have been explored as part of the Embodied Question Answering (EQA) task~\cite{das2018embodied}. The original EQA work~\cite{} and its subsequent studies~\cite{} define the task as involving four major components: (1) scene exploration, (2) scene memorization, (3) commonsense reasoning, and (4) localization and perception for answering questions. Most recent studies focus on the first two components and often leverage large language or vision–language models for the third. These components mainly correspond to distinct research areas: exploration relates to planning in robotics, memorization to representation learning, and reasoning to language understanding. In contrast, the fourth component, active perception, represents the core computer vision problem, where the agent must move, look, and perceive actively to gather visual information necessary to answer a question. In this work, we focus on this last component and provide a concrete setup.

Compared to previous active perception studies, we concretize our problem setup and propose an advanced systems mainly in three asepect. First, rather than only learning only the agent’s position in the scene as shown in many previous work~\cite{}, we explicitly aim to learn the optimal \emph{viewpoint} for answering the question. To achieve this, we consider the full set of control parameters of a typical mobile agent: heading rotation, forward translation, and view rotation.

Second, we pursue fine-grained control over these motion parameters rather than discretizing them into coarse categories such as left, right, forward, or backward, as done in previous work~\cite{}. Our model instead predicts continuous quantities—for example, rotation angles (in degrees) and translation distances (in centimeters), allowing for precise and adaptive viewpoint adjustment. Such fine-grained actions were largely infeasible in prior EQA frameworks, which relied on multi-turn navigation and sparse-reward settings primarily designed for exploration and memorization. By narrowing our focus to single-step active view selection, which can be learned without assuming multi-turn sequences during inference, we make it feasible to train continuous, high-resolution control policies.

Finally, and most importantly, unlike previous zero-shot EQA approaches~\cite{} that rely solely on the pretrained capabilities of large VLMs, we propose a learning-based active perception framework and demonstrate its strong generalization to unseen environments. For training, we curate synthetic datasets built upon CLEVR~\cite{} and ProTHOR~\cite{}, collectively referred to as XXX. Each dataset consists of paired query and target views. The query view is designed to partially include objects visible in the target view while omitting others, thereby simulating incomplete visual observations. Correspondingly, a question prompt is generated to ask about the missing information, requiring the agent to infer and predict the appropriate mobility parameters necessary to move from the query view to the target viewpoint.

To fine-tune pretrained VLMs for this task, we explore two strategies: supervised fine-tuning (SFT), which directly learns the parameters to reach the ground-truth view using an $\ell_2$ regression loss, and GRPO-based unsupervised fine-tuning, where the model predicts the mobility parameters at the end of its reasoning process without explicit supervision. By combining the advantages of both, we propose a sequential SFT-then-GRPO training strategy, which first grounds the model through supervised learning and then refines it through unsupervised policy optimization. This hybrid approach improves both performance and generalization to unseen environments.

In our experiments, our results demonstrate that training-based methods substantially outperform zero-shot approaches in Active View Selection(AVS)–based question answering, confirming the effectiveness of learning active visual perception beyond the pretrained capabilities of existing VLMs.


%In contrast, many previous EQA works focus only on locomotion, where the agent learns to reach a target location but not to choose the most informative view.
%In our experiments, we demonstrate that incorporating our view adaptation module into existing EQA pipelines consistently improves task performance.
%partially observable Markov decision process (POMDP) problems
%As expected, SFT achieves higher training accuracy but tends to overfit the training data, whereas GRPO yields better generalization at the cost of slightly lower overall performance. 

==> tables/backup/existing_eqa_benchmark.tex <==
% \begin{table*}[t!]
%     \footnotesize
%     \centering
%     \caption{Comprehensive comparison of our method with EQA frameworks across various backbone models and benchmarks. For each benchmark, we report baseline performance (Base) and results with our method as a plugin (+Ours). The best performance in each category is in \textbf{bold} and second best is \underline{underlined}.}
%     \label{tab:eqa_comprehensive_comparison}

%     % Column layout: 8 (ExpressBench) + 3 (SAT)
%     \begin{tabularx}{\linewidth}{l *{6}{Y} | Y | *{3}{Y}}
%         \toprule

%         % --- Group Header Row ---
%         \multicolumn{8}{c}{\textbf{Fine-EQA Benchmark}~\cite{Liu:2024EXPRESSBench}} 
%         & \multicolumn{3}{|c}{\textbf{SAT}~\cite{Ray:2024SAT}} \\
%         \midrule

%         % --- Sub-column Headers ---
%         \textbf{Method} & \textbf{Attribute} & \textbf{Counting} & \textbf{Existence} & 
%         \textbf{Object} & \textbf{State} & \textbf{Location} & \textbf{Average} &
%         \textbf{Method} & \textbf{Synthetic} & \textbf{Real} \\
%         \midrule

%         % ========== ROWS ==========

%         Fine-EQA~\cite{Liu:2024EXPRESSBench} &
%         49.23 & 38.75 & 67.92 & \textbf{57.41} & \underline{63.20} & 41.14 & 52.94 &
%         Base & \underline{59.11} & 60.00 \\

%         w/ SFT &
%         \textbf{59.08} & 45.00 & 67.29 & \underline{56.30} & 58.40 & \underline{45.71} & \underline{55.30} &
%         + SFT & \textbf{69.33} & \underline{67.33} \\

%         w/ RL &
%         52.00 & 44.38 & \textbf{69.17} & 47.41 & 62.00 & 42.29 & 52.87 &
%         + RL & 57.31 & 57.33 \\

%         \textbf{w/ Ours} &
%         \underline{53.23} & \textbf{52.50} & \underline{68.13} & 55.93 & \textbf{65.40} & \textbf{50.86} & \textbf{57.67} &
%         + Ours & \textbf{69.33} & \textbf{77.33} \\

%         \bottomrule
%     \end{tabularx}
% \end{table*}


% \begin{table*}[t!]
%     \footnotesize
%     \centering
%     \caption{Comprehensive comparison of our method with EQA frameworks across Fine-EQA and SAT benchmarks.}
%     \label{tab:eqa_comprehensive_comparison}

%     \begin{minipage}{0.62\linewidth}
%         \centering
%         \textbf{Fine-EQA Benchmark}~\cite{Liu:2024EXPRESSBench}

%         \begin{tabularx}{\linewidth}{l *{6}{Y} Y}
%             \toprule
%             \textbf{Method} &
%             \textbf{Attribute} & \textbf{Counting} & \textbf{Existence} &
%             \textbf{Object} & \textbf{State} & \textbf{Location} & \textbf{Avg} \\
%             \midrule

%             Fine-EQA~\cite{Liu:2024EXPRESSBench} &
%             49.23 & 38.75 & 67.92 & \textbf{57.41} & \underline{63.20} & 41.14 & 52.94 \\

%             w/ SFT &
%             \textbf{59.08} & 45.00 & 67.29 & \underline{56.30} & 58.40 & \underline{45.71} & \underline{55.30} \\

%             w/ RL &
%             52.00 & 44.38 & \textbf{69.17} & 47.41 & 62.00 & 42.29 & 52.87 \\

%             \textbf{w/ Ours} &
%             \underline{53.23} & \textbf{52.50} & \underline{68.13} & 55.93 & \textbf{65.40} & \textbf{50.86} & \textbf{57.67} \\
%             \bottomrule
%         \end{tabularx}
%     \end{minipage}
%     \hfill
%     \begin{minipage}{0.35\linewidth}
%         \centering
%         \textbf{SAT Benchmark}~\cite{Ray:2024SAT}

%         \begin{tabularx}{\linewidth}{l *{2}{Y}}
%             \toprule
%             \textbf{Method} & \textbf{Synthetic} & \textbf{Real} \\
%             \midrule

%             Base & \underline{59.11} & 60.00 \\
%             + SFT & \textbf{69.33} & \underline{67.33} \\
%             + RL & 57.31 & 57.33 \\
%             + Ours & \textbf{69.33} & \textbf{77.33} \\
%             \bottomrule
%         \end{tabularx}
%     \end{minipage}


% \end{table*}


% \begin{table*}[t!]
%     \footnotesize
%     \centering
%     \caption{Comprehensive comparison of our method with EQA frameworks across Fine-EQA and SAT benchmarks.}
%     \label{tab:eqa_comprehensive_comparison}

%     \begin{subtable}[t]{0.62\linewidth}
%         \centering
%         \caption{Fine-EQA Benchmark~\cite{Liu:2024EXPRESSBench}}
%         \label{tab:fine_eqa}

%         \begin{tabularx}{\linewidth}{l *{6}{Y} Y}
%             \toprule
%             \textbf{Method} &
%             \textbf{Attribute} & \textbf{Counting} & \textbf{Existence} &
%             \textbf{Object} & \textbf{State} & \textbf{Location} & \textbf{Avg} \\
%             \midrule

%             Fine-EQA~\cite{Liu:2024EXPRESSBench} &
%             49.23 & 38.75 & 67.92 & \textbf{57.41} & \underline{63.20} & 41.14 & 52.94 \\

%             w/ SFT &
%             \textbf{59.08} & 45.00 & 67.29 & \underline{56.30} & 58.40 & \underline{45.71} & \underline{55.30} \\

%             w/ RL &
%             52.00 & 44.38 & \textbf{69.17} & 47.41 & 62.00 & 42.29 & 52.87 \\

%             \textbf{w/ Ours} &
%             \underline{53.23} & \textbf{52.50} & \underline{68.13} & 55.93 & \textbf{65.40} & \textbf{50.86} & \textbf{57.67} \\
%             \bottomrule
%         \end{tabularx}
%     \end{subtable}
%     \hfill
%     \begin{subtable}[t]{0.35\linewidth}
%         \centering
%         \caption{SAT Benchmark~\cite{Ray:2024SAT}}
%         \label{tab:sat}

%         \begin{tabularx}{\linewidth}{l *{2}{Y}}
%             \toprule
%             \textbf{Method} & \textbf{Synthetic} & \textbf{Real} \\
%             \midrule

%             Base & \underline{59.11} & 60.00 \\
%             SFT & \textbf{69.33} & \underline{67.33} \\
%             RL & 57.31 & 57.33 \\
%             \textbf{SFT+RL (Ours}) & \textbf{69.33} & \textbf{77.33} \\
%             \bottomrule
%         \end{tabularx}
%     \end{subtable}
% \end{table*}

\begin{table*}[t!]
\centering
\setlength{\tabcolsep}{6pt}            % (optional) column padding
\renewcommand{\arraystretch}{1.15}     % (optional) row height

% ---------- Left table (Fine-EQA) ----------
\begin{minipage}[t]{0.63\linewidth}
  \centering
  \captionof{table}{\textbf{Comparison on Fine-EQA Benchmark.}
  Each column reports accuracy for a specific question type.
  Based on Fine-EQA~\cite{Liu:2024EXPRESSBench} framework, we compare different training strategies.
  Best is in \textbf{bold}, second best is \underline{underlined}.}
  \label{tab:fine_eqa_benchmark}
  {\scriptsize
  \begin{tabularx}{\linewidth}{l *{6}{Y} Y}
    \toprule
    \textbf{Method} &
    \textbf{Attribute} & \textbf{Counting} & \textbf{Existence} &
    \textbf{Object} & \textbf{State} & \textbf{Location} & \textbf{Average} \\
    \midrule

    Fine-EQA~\cite{Liu:2024EXPRESSBench} &
    49.23 & 38.75 & 67.92 & \textbf{57.41} & \underline{63.20} & 41.14 & 52.94 \\

    w/ SFT &
    \textbf{59.08} & 45.00 & 67.29 & \underline{56.30} & 58.40 & \underline{45.71} & \underline{55.30} \\

    w/ RL &
    52.00 & 44.38 & \textbf{69.17} & 47.41 & 62.00 & 42.29 & 52.87 \\

    \textbf{w/ Ours} &
    \underline{53.23} & \textbf{52.50} & \underline{68.13} & 55.93 &
    \textbf{65.40} & \textbf{50.86} & \textbf{57.67} \\
    \bottomrule
  \end{tabularx}}
\end{minipage}% 
\hfill
% ---------- Right table (SAT) ----------
\begin{minipage}[t]{0.35\linewidth}
  \centering
  \captionof{table}{\textbf{Results on SAT Benchmark.}
  We report performance both for synthetic and real splits.
  Best is in \textbf{bold}, second best is \underline{underlined}.}
  \label{tab:sat_benchmark}
  {\scriptsize
  \begin{tabularx}{\linewidth}{l *{2}{Y}}
    \toprule
    \textbf{Method} & \textbf{Synthetic} & \textbf{Real} \\
    \midrule

    Qwen2.5VL-7B~\cite{Bai:2025Qwen2.5VL}   & \underline{59.11} & 60.00 \\
    SFT  & \textbf{69.33} & \underline{67.33} \\
    RL   & 57.31 & 57.33 \\
    \textbf{SFT + RL (Ours)} & \textbf{69.33} & \textbf{77.33} \\
    \bottomrule
  \end{tabularx}}
\end{minipage}

\end{table*}


==> tables/backup/existing_eqa_benchmark_backup.tex <==
\begin{table*}[h!]
    \small
    \centering
    \caption{Comprehensive comparison of our method with EQA frameworks across various backbone models and benchmarks. For each benchmark, we report baseline performance (Base) and results with our method as a plugin (+Ours).}
    \label{tab:eqa_comprehensive_comparison}
    \definecolor{Gray}{gray}{0.9}
    
    \begin{tabularx}{\linewidth}{
        >{\raggedright\arraybackslash}p{3.2cm}
        Y Y Y Y Y Y Y
    }
    \toprule
    & \textbf{Attribute} & \textbf{Counting} & \textbf{Existence} & \textbf{Object} & \textbf{State} & \textbf{Location} & \textbf{Avg}
    \midrule
    % \multicolumn{7}{l}{\textbf{\textit{Explore-EQA Framework}}} \\
    % \addlinespace[0.5ex]
    % Prismatic-7B~\cite{Karamcheti:2024Prismatic}    & & & & & & \\
    % GPT-4o~\cite{OpenAI:2024GPT4o}                  & & & & & & \\
    % Qwen2.5-VL-7B~\cite{Bai:2025Qwen2.5VL}           & & & & & & \\
    % \addlinespace[1ex]
    % \midrule
    % \multicolumn{7}{l}{\textbf{\textit{Fine-EQA Framework}}} \\
    % \addlinespace[0.5ex]
    Fine-EQA~\cite{Liu:2024EXPRESSBench}    & -- & -- & -- & -- & -- & -- & -- \\
    w/ SFT only                             & -- & -- & -- & -- & -- & -- & -- \\
    w/ GRPO only                            & -- & -- & -- & -- & -- & -- & -- \\
    w/ Ours                                 & -- & -- & -- & -- & -- & -- & -- \\
    % \addlinespace[1ex]
    % \midrule
    % \multicolumn{7}{l}{\textbf{\textit{GraphEQA Framework}}} \\
    % \addlinespace[0.5ex]
    % Prismatic-7B~\cite{Karamcheti:2024Prismatic}    & & & & & & \\
    % Llama3-Mav~\cite{Dubey:2024Llama3}              & & & & & & \\
    % Qwen2.5-VL-7B~\cite{Bai:2025Qwen2.5VL}           & & & & & & \\
    \bottomrule
    \end{tabularx}
\end{table*}

==> tables/backup/existing_spatial_reasoning_benchmark.tex <==
\begin{table}[t]
\centering
\caption{Overall performance comparison on SAT~\cite{Ray:2024SAT} Benchmark.}
\label{tab:spatial_bench_overall}
\definecolor{Gray}{gray}{0.9}
\sisetup{detect-weight, mode=text}

\setlength{\tabcolsep}{4pt}
\scriptsize

\begin{tabular*}{\columnwidth}{l @{\extracolsep{\fill}} *6{S[table-format=1.3]}}
\toprule
 & {\textbf{Qwen-2.5-VL}~\cite{Bai:2025Qwen2.5VL}} &
   {\textbf{w/ SFT}} &
   {\textbf{w/ RL}} &
   {\textbf{w/ SFT + RL (Ours)}} \\
\midrule
\textbf{Overall} &
0.591 &
\textbf{0.699} &
0.573 &
\textbf{0.699} \\
\bottomrule
\end{tabular*}
\end{table}


==> tables/backup/existing_spatial_reasoning_benchmark_backup.tex <==
\begin{table*}[h!]
\centering
\caption{Performance comparison across Out-of-Domain spatial reasoning benchmarks (Part 1).}
\label{tab:spatial_bench_part1}
\definecolor{Gray}{gray}{0.9} % Define color for highlighting
\sisetup{detect-weight, mode=text} % siunitx setup

\begin{tabular}{l S[table-format=2.1] S[table-format=2.1] S[table-format=2.1] S[table-format=2.1]}
\toprule
\textbf{Model} & {\textbf{CV-Bench}} & {\textbf{SpatialRGPT}} & {\textbf{3DSRBench}} & {\textbf{CA-VQA}} \\
\midrule
GPT-4o~\cite{OpenAI:2024GPT4o} & & & & \\
Claude Sonnet 4~\cite{Anthropic:2024ClaudeSonnet4} & & & & \\
Gemini-2.5-Pro~\cite{Google:2024Gemini25} & & & & \\
Qwen-2.5-VL-7B~\cite{Bai:2025Qwen2.5VL} & & & & \\
\midrule
\rowcolor{Gray}
\textbf{Ours} & & & & \\
\bottomrule
\end{tabular}
\end{table*}

\begin{table*}[h]
\centering
\caption{Performance comparison across Out-of-Domain spatial reasoning benchmarks (Part 2).}
\label{tab:spatial_bench_part2}
\definecolor{Gray}{gray}{0.9} % Define color for highlighting
\sisetup{detect-weight, mode=text} % siunitx setup

\begin{tabular}{l S[table-format=2.1] S[table-format=2.1] S[table-format=2.1] S[table-format=2.1]}
\toprule
\textbf{Model} & {\textbf{RoboSpatial}} & {\textbf{EmbSpatial}} & {\textbf{SAT}} & {\textbf{BLINK}} \\
\midrule
GPT-4o~\cite{OpenAI:2024GPT4o} & & & & \\
Claude Sonnet 4~\cite{Anthropic:2024ClaudeSonnet4} & & & & \\
Gemini-2.5-Pro~\cite{Google:2024Gemini25} & & & & \\
Qwen-2.5-VL-7B~\cite{Bai:2025Qwen2.5VL} & & & & \\
\midrule
\rowcolor{Gray}
\textbf{Ours} & & & & \\
\bottomrule
\end{tabular}
\end{table*}


==> tables/backup/vgavs_main_backup.tex <==
% \definecolor{opensourcecolor}{HTML}{cdb4db}
% \definecolor{spatialcolor}{HTML}{ffc8dd}
% \definecolor{eqacolor}{HTML}{ffafcc}
% \definecolor{procolor}{HTML}{bde0fe}
% \definecolor{ourscolor}{HTML}{a2d2ff}

% \definecolor{opensourcecolor}{HTML}{f19c79}
% \definecolor{spatialcolor}{HTML}{ffe1a8} 
% \definecolor{eqacolor}{HTML}{f6f4d2}
% \definecolor{procolor}{HTML}{cbdfbd}
% \definecolor{ourscolor}{HTML}{d4e09b}

\definecolor{opensourcecolor}{HTML}{0072B2} 
\definecolor{spatialcolor}{HTML}{E69F00}   
\definecolor{eqacolor}{HTML}{009E73}      
\definecolor{procolor}{HTML}{D55E00}     
\definecolor{ourscolor}{HTML}{cbdfbd}     


\begin{table*}[h!]
    \centering
    \footnotesize
    \caption{Performance comparison on our proposed \Benchmark{} benchmark. We report scores for each category and the overall average. For \Benchmark{}-HM3D, we report LLM-scores originally rated on a 1–5 scale and linearly normalized to percentages. The best performance (except for \textit{`No Action'} category) in each category is in \textbf{bold} and second best is \underline{underlined}. For the internal comparison, we trained the model for 7 epochs for SFT and 5 epochs for GRPO in default.}
    \label{tab:last_mile_vqa_results_final}
    \setlength{\tabcolsep}{2pt}
    % Define a light gray color for highlighting 'Ours'
    \definecolor{Gray}{gray}{0.9}
    % Setup for siunitx columns, assuming scores are like XX.X
    % \sisetup{detect-weight, mode=text}
    \begin{tabularx}{\linewidth}{
        >{\raggedright\arraybackslash}p{2.4cm} >{\raggedright\arraybackslash}p{2.5cm} |
        Y Y Y | Y |  % ProcTHOR: Ex, Cnt, State | Average
        Y Y Y Y Y | Y  % HM3D: Attr, Ex, Cnt, Obj, State | Average
    }
    \toprule
    \multicolumn{2}{c|}{\multirow{2}{*}{\textbf{Action Model}}}  & \multicolumn{4}{c|}{\Benchmark{}-\textbf{ProcTHOR}~\cite{Deitke:2022ProcTHOR}} & \multicolumn{6}{c}{\Benchmark{}-\textbf{HM3D}~\cite{Ramakrishnan:2021HM3D}} \\
    \cmidrule(lr){3-6}\cmidrule(lr){7-12}
    & & \scriptsize{\textbf{Existence}} & \scriptsize{\textbf{Counting}} & \scriptsize{\textbf{State}} & \scriptsize{\textbf{Average}} 
    & \scriptsize{\textbf{Attribute}} & \scriptsize{\textbf{Existence}} & \scriptsize{\textbf{Counting}} & \scriptsize{\textbf{Object}} & \scriptsize{\textbf{State}} & \scriptsize{\textbf{Average}} \\
    \midrule
    %\hline
    %& \rowcolor{Gray}\textbf{\textit{No Action}} & \multicolumn{10}{c}{} \\
    %\addlinespace[0.5ex]
    \multirow{2}{*}{\textbf{No Action}}& \rowcolor{Gray}Query view        & 49.22 & 16.36 & 61.57 & 42.38 & 66.67 & 56.15 & 67.50 & 48.33 & 54.59 &  58.65\\
    & \rowcolor{Gray}Target view       & 93.02 & 69.14 & 92.58 & 84.91 & 74.48 & 77.50 & 86.67 & 71.79 & 80.00 & 78.09 \\
    \midrule
    %\hline
    % \rowcolor{opensourcecolor!18}\textbf{\textit{Open-Source Models}} & \multicolumn{10}{c}{} \\
    %\addlinespace[0.5ex]
    \textbf{Backbone} & \cellcolor{opensourcecolor!18} Qwen2.5-VL-7B~\cite{Bai:2025Qwen2.5VL}            & 64.34 & 29.74 & 56.55 & 50.21 & 49.17  & 46.15 & 66.25 & 46.86 & 66.49 & 54.98 \\
    % LLaVA-OV-1.5-8B~\cite{Li:2024LLaVAOneVision}      & & & & & \\
    % InternVL3-8B~\cite{Chen:2024InternVL3}            & & & & & \\
    % \addlinespace[1ex]
    \midrule
    %\hline
    % \multicolumn{5}{l}{\textbf{\textit{Spatial VLMs}}} \\
    %\addlinespace[0.5ex]
    % \rowcolor{spatialcolor!18}\textbf{\textit{Spatial VLMs}} & \multicolumn{10}{c}{} \\
    \addlinespace[0.5ex]
    \multirow{2}{*}{\textbf{Spatial VLMs}} & \cellcolor{spatialcolor!18}ViLaSR~\cite{Junfei:2025VILASR}                   & 57.95 & 25.46 & 52.84 & 45.42 & 50.00 & 48.46 & 68.33 & 50.00 & 52.70 & 53.90 \\
    & \cellcolor{spatialcolor!18}SpatialReasoner~\cite{Ma:2025SpatialReasoner}          & 54.65 & 22.68 & 52.62 & 43.32 & 37.50 & 50.00 & 70.42 & 40.00 & 47.30 & 49.04 \\
    % \addlinespace[1ex]
    \midrule
    %\hline
    %\multicolumn{5}{l}{\textbf{\textit{EQA Frameworks}}} \\
    %\addlinespace[0.5ex]
    %\rowcolor{eqacolor!18}\textbf{\textit{EQA Frameworks}} & \multicolumn{10}{c}{}\\
    \addlinespace[0.5ex]
    \textbf{EQA Methods} & \cellcolor{eqacolor!18}Fine-EQA~\cite{Liu:2024EXPRESSBench}                   & 63.57 & 31.97 & 64.41 & 53.32 & 54.17 & 52.31 & 70.00 & 44.44 & 52.70 & 54.72 \\
    \midrule
    %\hline
    %\multicolumn{5}{l}{\textbf{\textit{Proprietary Models}}} \\
    %\addlinespace[0.5ex]
    % \rowcolor{procolor!18}\textbf{\textit{Proprietary Models}} & \multicolumn{10}{c}{} \\
    \addlinespace[0.5ex]
    \multirow{2}{*}{\textbf{Proprietary}} & \cellcolor{procolor!18}GPT-5~\cite{OpenAI:2025GPT5}                    & 81.01 & 55.58 & 79.69 & 72.09 & 65.83 & 54.62 & 76.67 & 60.00 & 65.95 & 64.91 \\
    & \cellcolor{procolor!18}Gemini-2.5-Pro~\cite{Google:2025Gemini25}         & 82.95 & 52.79 & 81.00 & 72.25 & 64.17 & 59.23 & 74.17 & 60.00 & 60.81 & 63.67 \\
    %\addlinespace[1ex]
    \midrule
    %\hline
    %\multicolumn{1}{l}{\textbf{\textit{Training Strategies}}} & \multicolumn{10}{c}{} \\
    %\addlinespace[0.5ex]
    % \cellcolor{ourscolor}\textbf{\textit{Training Strategies}} & \multicolumn{10}{l}{}\\
    % & \rowcolor{ourscolor}\textbf{\textit{AVS Frameworks}} & \multicolumn{10}{c}{Backbone Model: Qwen2.5-VL-7B~\cite{Bai:2025Qwen2.5VL}} \\ 
    \addlinespace[0.5ex]
    % \midrule
    \multirow{7}{*}{\makecell[l]{\textbf{AVS Frameworks}\\(Backbone:\\Qwen2.5-VL-7B~\cite{Bai:2025Qwen2.5VL})}} & \cellcolor{ourscolor}SFT               & \underline{91.28} & 57.06 & 83.84 & 77.39 & 66.67 & \underline{70.77} & 67.50 & 55.56 & 62.16 & 64.53 \\
    & \cellcolor{ourscolor}SFT w/ NT Loss~\cite{Zausinger:2025NTLoss}               & 81.59 & 60.41 & 77.51 & 73.17 & 60.83 & 70.00 & 77.08 & \textbf{63.89} & 63.24 & 67.01 \\
    & \cellcolor{ourscolor}SFT (extended)              & 91.28 & 61.52 & \underline{85.59} & \underline{79.46} & \textbf{73.33} & 67.69 & 76.67 & 55.56 & 68.92 & 68.43\\
    & \cellcolor{ourscolor}RL             & 86.82 & \underline{65.24} & 83.41 & 78.49 & 69.17 & 70.00 & \textbf{81.25} & 60.00 & \underline{72.97} & \underline{70.68} \\
    & \cellcolor{ourscolor}RL w/ $r^{\text{pose}}$              & 86.05 & 61.52 & 83.41 & 76.99 & \underline{70.83} & 66.92 & \underline{78.33} & 58.89 & 72.43 & 69.48 \\
    & \cellcolor{ourscolor}\textbf{SFT+RL (Ours)}              & \textbf{91.47} & \textbf{69.52} & \textbf{90.17} & \textbf{83.72} & \underline{70.83} & \textbf{71.54}& 74.58 & \underline{62.78} & \textbf{73.78} & \textbf{70.70} \\
    %\cellcolor{ourscolor}\textbf{SFT+RL (Ours)}              & \textbf{91.47} & \textbf{69.52} & \textbf{90.17} & \textbf{83.72} & \underline{70.83} & \textbf{71.54}& 74.58 & \underline{62.78} & \textbf{73.78} & \textbf{70.70} \\
    \bottomrule
    %\hline
    \end{tabularx}
    \end{table*}
    


==> tables/supp_internal_comparison_backup.tex <==
% \definecolor{opensourcecolor}{HTML}{0072B2} 
% \definecolor{spatialcolor}{HTML}{E69F00}   
% \definecolor{eqacolor}{HTML}{009E73}      
% \definecolor{procolor}{HTML}{D55E00}     
% \definecolor{ourscolor}{HTML}{cbdfbd}     


\begin{table*}[h!]
    \centering
    \footnotesize
    \caption{\textbf{Quantitative comparison on internal baselines.} We report VQA accuracy on \Benchmark{}-ProcTHOR and LLM-Match scores on \Benchmark{}-HM3D, normalized to a percentage scale. The best except for \textit{`No Action'} in each column is in \textbf{bold} and second best is \underline{underlined}.}
    \label{tab:supp_internal_comparison}
    \vspace{-0.5\baselineskip}
    \setlength{\tabcolsep}{2pt}
    % Define a light gray color for highlighting 'Ours'
    \definecolor{Gray}{gray}{0.9}
    % Setup for siunitx columns, assuming scores are like XX.X
    % \sisetup{detect-weight, mode=text}
    \begin{tabularx}{\linewidth}{
        >{\raggedright\arraybackslash}p{2.4cm} >{\raggedright\arraybackslash}p{2.5cm} |
        Y Y Y | Y |  % ProcTHOR: Ex, Cnt, State | Average
        Y Y Y Y Y | Y  % HM3D: Attr, Ex, Cnt, Obj, State | Average
    }
    \toprule
    % \midrule
    \multirow{3}{*}{\makecell[l]{\textbf{AVS Framework}\\(Backbone:\\Qwen2.5-VL-7B~\cite{Bai:2025Qwen2.5VL})}} & SFT               & \underline{91.28} & 57.06 & \underline{83.84} & 77.39 & 67.50 & \underline{70.77} & 62.16 & 66.67 & 55.56 & 64.53 \\
    SFT (Extended) & \underline{91.28} & 57.06 & \underline{83.84} & 77.39 & 67.50 & \underline{70.77} & 62.16 & 66.67 & 55.56 & 64.53 \\
    SFT w/ NTLoss~\cite{Zausinger:2025NTLoss}           & \underline{91.28} & 57.06 & \underline{83.84} & 77.39 & 67.50 & \underline{70.77} & 62.16 & 66.67 & 55.56 & 64.53 \\
    & RL             & 86.82 & \underline{65.24} & 83.41 & \underline{78.49} & \textbf{81.25} & 70.00 & \underline{72.97} & \underline{69.17} & \underline{60.00}  & \underline{70.68} \\
    & RL w/ $r^\text{pose}$  & 86.82 & \underline{65.24} & 83.41 & \underline{78.49} & \textbf{81.25} & 70.00 & \underline{72.97} & \underline{69.17} & \underline{60.00}  & \underline{70.68} \\
    & \textbf{SFT+RL (Ours)}              & \textbf{91.47} & \textbf{69.52} & \textbf{90.17} & \textbf{83.72} & 74.58 & \textbf{71.54} & \textbf{73.78} & \textbf{70.83} & \textbf{62.78} & \textbf{70.70} \\
    \bottomrule
    \end{tabularx}
    \vspace{-\baselineskip}
\end{table*}
    


==> tables/supp_multiturn.tex <==
\begin{table}[t!]
    \centering
    \footnotesize
    \caption{\textbf{Quantitative comparison with multi-turn actions.} We report VQA accuracy on \Benchmark{}-ProcTHOR. The best in each column is in \textbf{bold} and second best is \underline{underlined}.}
    \label{tab:supp_multiturn}
    \setlength{\tabcolsep}{2pt}
    % Define a light gray color for highlighting 'Ours'
    \definecolor{Gray}{gray}{0.9}
    \begin{tabularx}{\linewidth}{
        >{\raggedright\arraybackslash}p{1.4cm} | >{\centering\arraybackslash}p{1.2cm} |
        Y Y Y | Y  % ProcTHOR: Ex, Cnt, State | Average
    }
    \toprule
    \multirow{2}{*}{{\makecell{\textbf{Training}\\\textbf{Variants}}}} & \multirow{2}{*}{{\makecell{\textbf{Action}\\\textbf{Steps}}}} & \multicolumn{4}{c}{\textbf{AVS-ProcTHOR}} \\
    \cmidrule(lr){3-6}
    & & \scriptsize{\textbf{Existence}} & \scriptsize{\textbf{Counting}} & \scriptsize{\textbf{State}} & \scriptsize{\textbf{Average}} \\
    \midrule
    \multirow{2}{*}{\makecell{SFT+RL\\(Q-only)}} & 1 & \textbf{91.47} & \textbf{69.52} & \underline{90.17} & \textbf{83.72} \\
                            & 2 & 87.60          & 61.52          & 87.55            & 78.89          \\
    % \midrule
    % \multirow{2}{*}{RL}     & 1 & 86.82          & 65.24          & 83.41            & 78.49          \\
                            % & 2 & 80.04          & 43.31          & 82.75            & 68.70          \\
    \midrule
    \multirow{2}{*}{\makecell{SFT+RL\\(Q+T)}} & 1 & \underline{90.50} & \underline{68.22} & \textbf{90.39}   & \underline{83.04} \\
                                                  & 2 & \underline{90.50} & \underline{68.22} & \underline{90.17} & 82.96         \\
    \bottomrule
    \end{tabularx}
    \vspace{-\baselineskip}
\end{table}

==> tables/vgavs_main_backup.tex <==
% \definecolor{opensourcecolor}{HTML}{cdb4db}
% \definecolor{spatialcolor}{HTML}{ffc8dd}
% \definecolor{eqacolor}{HTML}{ffafcc}
% \definecolor{procolor}{HTML}{bde0fe}
% \definecolor{ourscolor}{HTML}{a2d2ff}

% \definecolor{opensourcecolor}{HTML}{f19c79}
% \definecolor{spatialcolor}{HTML}{ffe1a8} 
% \definecolor{eqacolor}{HTML}{f6f4d2}
% \definecolor{procolor}{HTML}{cbdfbd}
% \definecolor{ourscolor}{HTML}{d4e09b}

\definecolor{opensourcecolor}{HTML}{0072B2} 
\definecolor{spatialcolor}{HTML}{E69F00}   
\definecolor{eqacolor}{HTML}{009E73}      
\definecolor{procolor}{HTML}{D55E00}     
\definecolor{ourscolor}{HTML}{cbdfbd}     


\begin{table*}[h!]
    \centering
    \footnotesize
    \caption{\textbf{Performance comparison on our proposed \Benchmark{} benchmark.} We report scores for each category and the overall average. For \Benchmark{}-HM3D, we report LLM-scores originally rated on a 1–5 scale and linearly normalized to percentages. The best performance (except for \textit{`No Action'} category) in each category is in \textbf{bold} and second best is \underline{underlined}.}
    \label{tab:vgavs_main}
    \vspace{-0.5\baselineskip}
    \setlength{\tabcolsep}{2pt}
    % Define a light gray color for highlighting 'Ours'
    \definecolor{Gray}{gray}{0.9}
    % Setup for siunitx columns, assuming scores are like XX.X
    % \sisetup{detect-weight, mode=text}
    \begin{tabularx}{\linewidth}{
        >{\raggedright\arraybackslash}p{2.4cm} >{\raggedright\arraybackslash}p{2.5cm} |
        Y Y Y | Y |  % ProcTHOR: Ex, Cnt, State | Average
        Y Y Y Y Y | Y  % HM3D: Attr, Ex, Cnt, Obj, State | Average
    }
    \toprule
    \multicolumn{2}{c|}{\multirow{2}{*}{\textbf{Action Model}}}  & \multicolumn{4}{c|}{\Benchmark{}-\textbf{ProcTHOR}~\cite{Deitke:2022ProcTHOR}} & \multicolumn{6}{c}{\Benchmark{}-\textbf{HM3D}~\cite{Ramakrishnan:2021HM3D}} \\
    \cmidrule(lr){3-6}\cmidrule(lr){7-12}
    & & \scriptsize{\textbf{Existence}} & \scriptsize{\textbf{Counting}} & \scriptsize{\textbf{State}} & \scriptsize{\textbf{Average}} 
    & \scriptsize{\textbf{Existence}} & \scriptsize{\textbf{Counting}} & \scriptsize{\textbf{State}} & \scriptsize{\textbf{Attribute}} & \scriptsize{\textbf{Object}} & \scriptsize{\textbf{Average}} \\
    \midrule
    %\hline
    %& \rowcolor{Gray}\textbf{\textit{No Action}} & \multicolumn{10}{c}{} \\
    %\addlinespace[0.5ex]
    \multirow{2}{*}{\textbf{No Action}}& \rowcolor{Gray}Query view        & 49.22 & 16.36 & 61.57 & 42.38 & 56.15 & 67.50 & 54.59 & 66.67 & 48.33 &  58.65\\
    & \rowcolor{Gray}Target view       & 93.02 & 69.14 & 92.58 & 84.91 & 77.50 & 86.67 & 80.00 & 74.48 & 71.79  & 78.09 \\
    \midrule
    \textbf{Backbone Model} & \cellcolor{opensourcecolor!18} Qwen2.5-VL-7B~\cite{Bai:2025Qwen2.5VL}            & 64.34 & 29.74 & 56.55 & 50.21  & 46.15 & 66.25 & 66.49 & 49.17 & 46.86 & 54.98 \\
    \midrule
    \addlinespace[0.5ex]
    \multirow{2}{*}{\textbf{Spatial VLMs}} & \cellcolor{spatialcolor!18}ViLaSR~\cite{Junfei:2025VILASR}                   & 57.95 & 25.46 & 52.84 & 45.42 & 48.46 & 68.33 & 52.70 & 50.00 & 50.00 & 53.90 \\
    & \cellcolor{spatialcolor!18}SpatialReasoner~\cite{Ma:2025SpatialReasoner}          & 54.65 & 22.68 & 52.62 & 43.32 & 50.00 & 70.42 & 47.30 & 37.50 & 40.00 & 49.04 \\
    % \addlinespace[1ex]
    \midrule
    %\hline
    %\multicolumn{5}{l}{\textbf{\textit{EQA Frameworks}}} \\
    %\addlinespace[0.5ex]
    %\rowcolor{eqacolor!18}\textbf{\textit{EQA Frameworks}} & \multicolumn{10}{c}{}\\
    \addlinespace[0.5ex]
    \textbf{EQA Framework} & \cellcolor{eqacolor!18}Fine-EQA~\cite{Liu:2024EXPRESSBench}                   & 63.57 & 31.97 & 64.41 & 53.32 & 52.31 & 70.00 & 52.70 & 54.17 & 44.44 & 54.72 \\
    \midrule
    %\hline
    %\multicolumn{5}{l}{\textbf{\textit{Proprietary Models}}} \\
    %\addlinespace[0.5ex]
    % \rowcolor{procolor!18}\textbf{\textit{Proprietary Models}} & \multicolumn{10}{c}{} \\
    \addlinespace[0.5ex]
    \multirow{2}{*}{\textbf{Proprietary Models}} & \cellcolor{procolor!18}GPT-5~\cite{OpenAI:2025GPT5}                    & 81.01 & 55.58 & 79.69 & 72.09 & 54.62 & \underline{76.67} & 65.95 & 65.83 & 60.00 & 64.91 \\
    & \cellcolor{procolor!18}Gemini-2.5-Pro~\cite{Google:2025Gemini25}         & 82.95 & 52.79 & 81.00 & 72.25 & 59.23 & 74.17 & 60.81 & 64.17 & 60.00 & 63.67 \\
    %\addlinespace[1ex]
    \midrule
    \addlinespace[0.5ex]
    % \midrule
    \multirow{3}{*}{\makecell[l]{\textbf{AVS Framework}\\(Backbone:\\Qwen2.5-VL-7B~\cite{Bai:2025Qwen2.5VL})}} & \cellcolor{ourscolor}SFT               & \underline{91.28} & 57.06 & \underline{83.84} & 77.39 & \underline{70.77} & 67.50 & 62.16 & 66.67 & 55.56 & 64.53 \\
    %& \cellcolor{ourscolor}SFT w/ NT Loss~\cite{Zausinger:2025NTLoss}               & 81.59 & 60.41 & 77.51 & 73.17 & 60.83 & 70.00 & 77.08 & \textbf{63.89} & 63.24 & 67.01 \\
    %& \cellcolor{ourscolor}SFT (extended)              & 91.28 & 61.52 & \underline{85.59} & \underline{79.46} & \textbf{73.33} & 67.69 & 76.67 & 55.56 & 68.92 & 68.43\\
    & \cellcolor{ourscolor}RL             & 86.82 & \underline{65.24} & 83.41 & \underline{78.49} & 70.00 & \textbf{81.25} & \underline{72.97} & \underline{69.17} & \underline{60.00}  & \underline{70.68} \\
    %& \cellcolor{ourscolor}RL w/ $r^{\text{pose}}$              & 86.05 & 61.52 & 83.41 & 76.99 & \underline{70.83} & 66.92 & \underline{78.33} & 58.89 & 72.43 & 69.48 \\
    & \cellcolor{ourscolor}\textbf{SFT+RL (Ours)}              & \textbf{91.47} & \textbf{69.52} & \textbf{90.17} & \textbf{83.72} & \textbf{71.54} & 74.58 & \textbf{73.78} & \textbf{70.83} & \textbf{62.78} & \textbf{70.70} \\
    %\cellcolor{ourscolor}\textbf{SFT+RL (Ours)}              & \textbf{91.47} & \textbf{69.52} & \textbf{90.17} & \textbf{83.72} & \underline{70.83} & \textbf{71.54}& 74.58 & \underline{62.78} & \textbf{73.78} & \textbf{70.70} \\
    \bottomrule
    %\hline
    \end{tabularx}
    \vspace{-\baselineskip}
\end{table*}
    

